ProxQuant: Quantized Neural Networks via Proximal Operators

To make deep neural networks feasible in resource-constrained environments (such as mobile devices), it is beneficial to quantize models by using low-precision weights. One common technique for quantizing neural networks is the straight-through gradient method, which enables back-propagation through the quantization mapping. Despite its empirical success, little is understood about why the straight-through gradient method works. Building upon a novel observation that the straight-through gradient method is in fact identical to the well-known Nesterov's dual-averaging algorithm on a quantization constrained optimization problem, we propose a more principled alternative approach, called ProxQuant, that formulates quantized network training as a regularized learning problem instead and optimizes it via the prox-gradient method. ProxQuant does back-propagation on the underlying full-precision vector and applies an efficient prox-operator in between stochastic gradient steps to encourage quantizedness. For quantizing ResNets and LSTMs, ProxQuant outperforms state-of-the-art results on binary quantization and is on par with state-of-the-art on multi-bit quantization. For binary quantization, our analysis shows both theoretically and experimentally that ProxQuant is more stable than the straight-through gradient method (i.e. BinaryConnect), challenging the indispensability of the straight-through gradient method and providing a powerful alternative.

==> Sections/convergence-thm.tex <==
\section{Impact of lazy projection on convergence}
Recall that prox-gradient algorithms (both lazy and non-lazy) aim to solve the problem
\begin{equation}
  \label{problem:regularized}
  \minimize_{\theta\in\R^d} L(\theta) + \lambda R(\theta).
\end{equation}
Without convexity of $L$ and $R$, one could only hope for convergence to stataionary points.

In this section, we perform a theoretical study on the impact of lazy projection on convergence. We show in Section~\ref{appendix:convergence-pq} that our \pq~algorithm (i.e. non-lazy prox-gradient method) converges under mild smoothness assumptions on the problem. In Section~\ref{appendix:nonconvergence-lazy}, we provide a simple example showing that the lazy prox-gradient method fails to converge under the same set of assumptions. This demonstrates the superiority of our proposed \pq~over lazy prox-gradient type algorithms such as the BinaryRelax~\citep{YinZhLyOsQiXi18}.

\subsection{A convergence theorem for \pq}
\label{appendix:convergence-pq}
% \yb{A tentative convergence theorem for \pq}.
We give a convergence theorem for \pq~under the assumption that the loss and regularizers are both smooth. We consider \pq~with batch gradient and constant regularization strength $\lambda_t\equiv \lambda$:
\begin{equation*}
  \theta_{t+1} = \prox_{\eta_t\lambda R}(\theta_t - \eta_t\grad L(\theta_t)).
\end{equation*}

Recall that a function $f:\R^d\to\R$ is said to be $\beta$-smooth if it is differentiable and $\grad f$ is $\beta$-Lipschitz: for all $x,y\in\R^d$ we have
\begin{equation*}
  \ltwo{\grad f(x) - \grad f(y)} \le \beta\ltwo{x-y}.
\end{equation*}
For any $\beta$-smooth function, it satisfies the bound
\begin{equation*}
  f(y) \le f(x) + \<\grad f(x), y-x\> + \frac{\beta}{2}\ltwo{x-y}^2~~~{\rm for~all}~x,y\in\R^d.
\end{equation*}
\begin{theorem}[Convergence of ProxQuant]
  \label{theorem:convergence-pq}
  Assume that the loss $L$ is $\beta$-smooth and the regularizer $R$
  is differentiable. Let
  $F_\lambda(\theta)=L(\theta)+\lambda R(\theta)$ be the composite
  objective and assume that it is bounded below by $F_\star$. Running
  ProxQuant with batch gradient $\grad L$, constant stepsize
  $\eta_t \equiv \eta = \frac{1}{2\beta}$ and
  $\lambda_t\equiv \lambda$ for $T$ steps, we have the convergence
  guarantee
  \begin{equation}
    \label{equation:convergence-pq}
    \ltwo{\grad F_\lambda(\theta_{T_{\rm best}})}^2 \le
    \frac{C\beta(F_\lambda(\theta_0) - F_\star)}{T}~~~{\rm
      where}~~~T_{\rm best} = \argmin_{1\le t\le T} \ltwo{\theta_t - \theta_{t-1}},
  \end{equation}
  where $C>0$ is a universal constant.
\end{theorem}

\begin{remark}
  The convergence guarantee requires both the loss and the regularizer
  to be smooth. For the loss, this can be satisfied if we use a smooth
  activation function (such as $\tanh$). For the regularizer, the
  quantization-inducing regularizers we considered in
  Section~\ref{section:wasserstein-reg} are non-differentiable -- for
  example, the W-shaped regularizer
  $R(\theta)=\sum_{j=1}^d\min\set{|\theta_i-1|, |\theta_i+1|}$ is
  non-differentiable as it is ``pointy'' at $\set{\pm 1,0}$. However,
  we can use a smoothed version of them that is differentiable and
  point-wise arbitrarily close to $R$, which will satisfy the
  assumptions of Theorem~\ref{theorem:convergence-pq}.
  % For example, for binary quantization, the regularizer $R(\theta)=\sum_{i=1}^d (\theta_i^2-1)^2$ is smooth while promoting the $\theta_i$'s to be in $\set{\pm 1}$.
\end{remark}

% \yb{Adding a remark here.}

Convergence results like Theorem~\ref{theorem:convergence-pq} are
standard in the literature of proximal algorithms, where we have
convergence to stataionarity without convexity on either $L$ or $R$
but assuming smoothness. For completeness we provide a proof
below. Note that though the convergence is ergodic, the best index
$T_{\rm best}$ can be obtained in practice via monitoring the proximity
$\ltwo{\theta_t - \theta_{t-1}}$.

\begin{proof}
  Recall the ProxQuant iterate
  \begin{equation*}
    \theta_{t+1} = \argmin_{\theta\in\R^d} \left\{ L(\theta_t) +
      \<\theta-\theta_t, \grad L(\theta_t)\> +
      \frac{1}{2\eta}\ltwo{\theta - \theta_t}^2 + \lambda R(\theta)
    \right\}.
  \end{equation*}
  By the fact that $\theta_{t+1}$ minimizes the above objective and
  applying the smoothness of $L$, we get that
  \begin{align*}
    & \quad F_\lambda(\theta_t) = L(\theta_t) + \lambda R(\theta_t)
      \ge L(\theta_t) + \<\theta_{t+1}
      - \theta_t, \grad L(\theta_t)\> +
      \frac{1}{2\eta}\ltwo{\theta_{t+1} - \theta_t}^2 + \lambda
      R(\theta_{t+1}) \\
    & \ge L(\theta_{t+1}) + \left( \frac{1}{2\eta} - \frac{\beta}{2}
      \right)\ltwo{\theta_{t+1} - \theta_t}^2 + \lambda
      R(\theta_{t+1}) = F_\lambda(\theta_{t+1}) +
      \frac{\beta}{2}\ltwo{\theta_{t+1} - \theta_t}^2.
  \end{align*}
  Telescoping the above bound for $t=0,\dots,T-1$, we get that
  \begin{equation*}
    \sum_{t=0}^{T-1} \ltwo{\theta_{t+1} - \theta_t}^2 \le
    \frac{2(F_\lambda(\theta_0) - F_\lambda(\theta_T))}{\beta} \le
    \frac{2(F_\lambda(\theta_0) - F_\star)}{\beta}.
  \end{equation*}
  Therefore we have the proximity guarantee
  \begin{equation}
    \label{equation:proximity}
    \min_{0\le t\le T-1} \ltwo{\theta_{t+1} - \theta_t}^2 \le
    \frac{2(F_\lambda(\theta_0) - F_\star)}{\beta T}. 
  \end{equation}
  We now turn this into a stationarity guarantee. The first-order
  optimality condition for $\theta_{t+1}$ gives
  \begin{equation*}
    \grad L(\theta_t) + \frac{1}{\eta}(\theta_{t+1} - \theta_t) +
    \lambda \grad R(\theta_{t+1}) = 0.
  \end{equation*}
  Combining the above equality and the smoothness of $L$, we get
  \begin{align*}
    & \quad \ltwo{\grad F_\lambda(\theta_{t+1})} = \ltwo{\grad L(\theta_{t+1}) +
      \lambda\grad R(\theta_{t+1})} = \ltwo{\frac{1}{\eta}(\theta_t -
      \theta_{t+1}) + \grad L(\theta_{t+1}) - \grad L(\theta_t)} \\
    & \le \left( \frac{1}{\eta} + \beta\right) \ltwo{\theta_{t+1} -
      \theta_t} = 3\beta\ltwo{\theta_{t+1} - \theta_t}.
  \end{align*}
  Choosing $t=T_{\rm best}-1$ and applying the proximity
  guarantee~\cref{equation:proximity}, we get
  \begin{equation*}
    \ltwo{\grad F_\lambda(\theta_{T_{\rm best}})}^2 \le
    9\beta^2 \ltwo{\theta_{T_{\rm best}} - \theta_{T_{\rm best}-1}}^2 =
    9\beta^2 \min_{0\le t\le T-1} \ltwo{\theta_{t+1} - \theta_t}^2 \le
    \frac{18\beta(F_\lambda(\theta_0) - F_\star)}{T}.
  \end{equation*}
  This is the desired bound.
\end{proof}

\subsection{Non-convergence of lazy prox-gradient}
\label{appendix:nonconvergence-lazy}
The lazy prox-gradient algorithm (e.g. BinaryRelax~\citep{YinZhLyOsQiXi18}) for solving problem~\cref{problem:regularized} is a variant where the gradients are taken at proximal points but accumulated at the original sequence:
\begin{equation}
  \label{algorithm:lazy}
  \theta_{t+1} = \theta_t - \eta_t\grad L(\prox_{\lambda R}(\theta_t)).
\end{equation}
Convergence of the lazy prox-gradient algorithm~\cref{algorithm:lazy} is only known to hold for convex problems~\citep{Xiao10}; on smooth non-convex problems it generally does not converge even in an ergodic sense. Here we provide a concrete example in one-dimension that satisfies the assumptions in Theorem~\ref{theorem:convergence-pq} (so that \pq~converges ergodically) but lazy prox-gradient does not converge.

\begin{lemma}[Non-convergence of lazy prox-gradient]
  There exists $L$ and $R$ satisfying the assumptions of Theorem~\ref{theorem:convergence-pq} such that for any constant stepsize $\eta_t\equiv \eta\le \frac{1}{2\beta}$, there exists some specific initialization $\theta_0$ on which the lazy prox-gradient algorithm~\cref{algorithm:lazy}
  does not converge even in the ergodic sense of~\cref{equation:convergence-pq}.
\end{lemma}
% \begin{proof}
\begin{wrapfigure}{R}{0.3\textwidth}
  \centering
  \includegraphics[width=0.28\textwidth]{Figures/w-smooth.pdf}
  \caption{}
  %\caption{\small Loss $L(\theta)$ and regularizer $R(\theta)$ (with $\eps=0.2$).}
  \label{figure:w-smooth}
\end{wrapfigure}

\noindent{\it Proof.} Let our loss function $L:\R\to\R$ be the quadratic $L(\theta)=\frac{1}{2}\theta^2$ (so that $L$ is $\beta$-smooth with $\beta=1$). Let the regularizer $R:\R\to\R$ be a smoothed version of the W-shaped regularizer in~\cref{equation:binary-reg}, defined as (for $\eps\in(0, 1/2]$ being the smoothing radius)

  \begin{equation*}
    R(\theta) = \left\{
      \begin{aligned}
        & -\frac{1}{2\eps}\theta^2 + 1 - \eps, &~~~\theta \in [0, \eps) \\
        & -\theta + 1 - \frac{\eps}{2}, &~~~\theta \in [\eps, 1-\eps) \\
        & \frac{1}{2\eps}(\theta-1)^2, &~~~\theta \in [1-\eps, 1+\eps) \\
        & \theta - 1 - \frac{\eps}{2}, &~~~\theta \in [1+\eps, \infty) \\
      \end{aligned}
    \right.
  \end{equation*}
  and $R(-\theta)=R(\theta)$ for the negative part. See Figure~\ref{figure:w-smooth} for an illustration of the loss $L$ and the regularizer $R$ (with $\eps=0.2$).
  % \vspace{0.2cm}

  It is straightforward to see that $R$ is piecewise quadratic and differentiable on $\R$ by computing the derivatives at $\eps$ and $1\pm \eps$. Further, by elementary calculus, we can evaluate the prox operator in closed form: for all $\lambda\ge 1$, we have
  \begin{equation*}
    \prox_{\lambda R}(\theta) = \frac{\eps\theta+\lambda\sign(\theta)}{\eps+\lambda\sign(\theta)}~~~\textrm{for all}~|\theta|\le 1.
  \end{equation*}

  Now, suppose we run the lazy prox-gradient method with constant stepsize $\eta_t\equiv \eta\le \frac{1}{2\beta}=\frac{1}{2}$. For the specific initialization
  \begin{equation*}
    \theta_0 = \frac{\eta\lambda}{2\lambda + (2-\eta)\eps} \in (0, 1),
  \end{equation*}
  we have the equality $\prox_{\lambda R}(\theta_0) = \frac{2}{\eta}\theta_0$ and therefore the next lazy prox-gradient iterate is
  \begin{equation*}
    \theta_1 = \theta_0 - \eta\grad L(\prox_{\lambda R}(\theta_0)) = \theta_0 - \eta\grad L\left(\frac{2}{\eta}\theta_0\right) = \theta_0 - \eta\cdot \frac{2}{\eta}\theta_0 = -\theta_0.
  \end{equation*}
  As both $R$ and $L$ are even functions, a symmetric argument holds for $\theta_1$ from which we get $\theta_2=-\theta_1=\theta_0$. Therefore the lazy prox-gradient method ends up oscillating between two points:
  \begin{equation*}
    \theta_t = (-1)^t\theta_0.
  \end{equation*}
  On the other hand, it is straightforward to check that the only stationary points of $L(\theta)+\lambda R(\theta)$ are $0$ and $\pm\frac{\lambda}{\eps+\lambda}$, all not equal to $\pm\theta_0$. Therefore the sequence $\{\theta_t\}_{t\ge 0}$ does not have a subsequence with vanishing gradient and thus does not approach stationarity in the ergodic sense. \qed
% \end{proof}


==> Sections/experiment.tex <==
\section{Experiments}
\label{section:experiment}
We evaluate the performance of \pq~on two tasks: image classification
with ResNets, and language modeling with LSTMs. On both tasks, we show
that the default straight-through gradient method is not the only
choice, and our \pq~can achieve the same and often better results.

\subsection{Image classification on CIFAR-10}
\label{section:cifar-10}
\paragraph{Problem setup} We perform image classification on the
CIFAR-10 dataset, which contains 50000 training images and 10000 test
images of size 32x32. We apply a commonly used data augmentation
strategy (pad by 4 pixels on each side, randomly crop to 32x32, do a
horizontal flip with probability 0.5, and normalize). Our models are
ResNets~\citep{HeZhReSu16} of depth 20, 32, and 44 with weights
quantized to binary or ternary.

\paragraph{Method} We use \pq~with
regularizer~\cref{equation:binary-reg} in the binary case
and~\cref{equation:ternary-prox,equation:ternary-quantizer} in the
ternary case, which we respectively denote as PQ-B and PQ-T.  We use
the homotopy method $\lambda_t=\lambda\cdot t$ with $\lambda=10^{-4}$
as the regularization strength and Adam with constant learning rate
0.01 as the optimizer.
% As the prox operator does not strictly enforce quantizedness,

We compare with BinaryConnect (BC) for binary nets and Trained Ternary
Quantization (TTQ)~\citep{ZhuHaMaDa16} for ternary nets. For
BinaryConnect,
% we haven't found reported results with ResNets on
% CIFAR-10, and
we train with the recommended Adam optimizer with
learning rate decay~\citep{CourbariauxBeDa15} (initial learning rate
0.01, multiply by 0.1 at epoch 81 and 122), which we find leads to the
best result for BinaryConnect.

Both the baseline and our methods are initialized at the same
pre-trained full-precision nets (warm-start) for fair comparison. To
accelerate training in the final stage, we do a hard quantization
$\theta\mapsto\q(\theta)$ at epoch 400 and keeps training till the
600-th epoch to stabilize the BatchNorm layers.
% consistent with
% previous work~\citep{CourbariauxBeDa15,Sun18}.

\paragraph{Result} The top-1 classification errors are reported in
Table~\ref{table:cifar-10}. For binary nets, our \pq-Binary
consistently yields better results than BinaryConnect. For ternary
nets, our results are comparable with the reported results of
TTQ,\footnote{We note that our \pq-Ternary and TTQ are not strictly
  comparable: we have the advantage of using better initializations;
  TTQ has the advantage of a stronger quantizer: they train the
  quantization levels $(\theta^+,\theta^-)$ whereas our
  quantizer~\cref{equation:ternary-quantizer} pre-computes them from
  the current full-precision parameter.} and the best performance of
our method over 4 runs (from the same initialization) is slightly
better than TTQ.

\begin{table}[h!]
  \centering
  \caption{Top-1 classification error of quantized ResNets on
    CIFAR-10. Performance is reported in mean(std) over 4 runs, where
    for PQ-T we report in addition the best of 4 (Bo4).}
  \label{table:cifar-10}
  \begin{tabular}{|c|c||c|c||c|c|c|}
    \hline
    Model & Full-Precision & BC & PQ-B (ours) & TTQ & PQ-T
    (ours) & PQ-T (Bo4) \\  
    (Bits) & (32) & (1) & (1) & (2) & (2) & (2) \\
    \hline
    ResNet-20 & 8.06 & 9.49 (0.22) & {\bf 9.15} (0.21) & 8.87 & {\bf 8.40}
                                                                (0.13)
           & 8.22
    \\ 
    ResNet-32 & 7.25 & 8.66 (0.36) & {\bf 8.40} (0.23) & 7.63 & 7.65
                                                                (0.15)
           & 7.53
    \\
    ResNet-44 & 6.96 & 8.26 (0.24) & {\bf 7.79} (0.06) & 7.02 &
                                                                7.05 (0.08) & 6.98 \\
    ResNet-56 & 6.61 & - (-) & {\bf -} (-) & - & - (-) & - \\
    \hline
  \end{tabular}
\end{table}

% \subsubsection{Convergence plot}
% \label{section:tuning-lambda}
% Plot the regularizer against epoch for different reg rates. 

\subsection{Language modeling with LSTMs}
\label{section:lstm}
\paragraph{Problem setup} We perform language modeling with
LSTMs~\cite{HochreiterSc97} on the Penn Treebank (PTB)
dataset~\citep{MarcusMaSa93}, which contains 929K training tokens, 73K
validation tokens, and 82K test tokens. Our model is a standard
one-hidden-layer LSTM with embedding dimension 300 and hidden
dimension 300. We train quantized LSTMs with the encoder, transition
matrix, and the decoder quantized to $k$-bits for
$k\in\set{1,2,3}$. The quantization is performed in a row-wise
fashion, so that each row of the matrix has its own codebook
$\set{\alpha_1,\dots,\alpha_k}$.
% We use the alternating multi-bit
% (ALT) quantizer~\citep{XuYaLiOuCaWaZh18}, a powerful multi-bit
% quantization algorithm giving quantization of the
% form~\cref{equation:multi-bit-quant}.

\paragraph{Method}
We compare our multi-bit \pq~(\cref{equation:multi-bit-prox}) to the
state-of-the-art alternating minimization algorithm with
straight-through gradients~\citep{XuYaLiOuCaWaZh18}.
% Using the ALT quantizer, we compare two training
% dynamics: the straight-through gradient method
% of~ and our \pq.~
Training is initialized at a
pre-trained full-precision LSTM. We use the SGD optimizer with initial
learning rate 20.0 and decay by a factor of 1.2 when the validation
error does not improve over an epoch. We train for 80 epochs with
batch size 20, BPTT 30, dropout with probability 0.5, and clip the
gradient norms to $0.25$. The regularization rate $\lambda$ is tuned
by finding the best performance on the validation set. In addition to
multi-bit quantization, we also report the results for binary LSTMs
(weights in $\set{\pm 1}$), comparing BinaryConnect and our
\pq -Binary whose learning rates are tuned on an exponential grid. 

% Although our method focuses on quantizing weights, we are able to
% also quantize the activation, which in LSTMs is defined as
% mapping quantizing the state vector to $k$-bit in the forward
% pass and straight-through in the backward pass. We report results for
% both weight-only quantization and weight+activation quantization.
% \yb{Polish.}

\paragraph{Result}
We report the perplexity-per-word (PPW, lower is better) in
Table~\ref{table:ptb}. The performance of \pq~is comparable with the
Straight-through gradient method. On Binary LSTMs, \pq-Binary beats
BinaryConnect by a large margin. These results demonstrate that
\pq~offers a powerful alternative for training recurrent networks.

\begin{table}[h!]
  \centering
  \caption{PPW of quantized LSTM on Penn Treebank.}
  \label{table:ptb}
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    Method / Number of Bits & 1 & 2 & 3 & FP (32) \\
    % \hline
    % Refined + Straight-through & - & - & 100.3 & - & 91.3 & - & \\
    \hline
    BinaryConnect & 372.2 & - & - & \multirow{4}{*}{88.5} \\
    \cline{1-4}
    \pq-Binary (ours) & {\bf 288.5} & - & - & \\
    \cline{1-4}
    ALT Straight-through\footnotemark & 104.7 & 90.2 & 86.1 & \\
    \cline{1-4}
    %\hline
    ALT-\pq~(ours) & 106.2 & 90.0 & 87.2 & \\
    \hline
  \end{tabular}
\end{table}

\footnotetext{We thank~\citet{XuYaLiOuCaWaZh18} for sharing the
  implementation of this method through a personal
  communication. There is a very clever trick not mentioned in their
  paper: after computing the alternating quantization $\q_{\rm alt}(\theta)$,
  they multiply by a constant 0.3 before taking the gradient; in other
  words, their quantizer is a rescaled alternating quantizer:
  $\theta\mapsto 0.3\q_{\rm alt}(\theta)$. This scaling step gives a
  significant gain in performance -- without scaling the PPW is
  $\set{116.7, 94.3, 87.3}$ for $\set{1,2,3}$ bits. In contrast, our
  \pq~does not involve a scaling step and achieves better PPW than
  this unscaled ALT straight-through method.}


% \footnotemark
% \footnotetext{The PPW is 150 through a communication 
%   with~\citet{XuYaLiOuCaWaZh18}.}

==> Sections/fixed-point.tex <==
\section{Proof of Theorem~\ref{theorem:fixed-point}}
% Consider the BinaryConnect method with batch gradient descent:
% \begin{equation}
%   \label{equation:batch-bc}
%   \begin{aligned}
%   \theta_{t} &= \sign(h_t)\\
%   h_{t+1} &= h_t - \eta_t\grad L(\theta_t).
%   \end{aligned}
% \end{equation}

% \begin{definition}[Fixed points and the convergence]
% We say that $\theta\in\{-1,1\}^d$ is a \textbf{fixed point} of the BinaryConnect algorithm, if there exists $h\in\R^{d}$ such that when we take $h_0=h$ in the iterates \cref{equation:batch-bc}  $\theta_t = \theta$ for all $t  = 0,1,2,...$.
% We say that the BinaryConnect algorithm \textbf{converges} with an initialization $h_0\in\R^{d}$ if there exists $t\in \infty$ such that $\theta_t$ is a fixed point.
% \end{definition}
% \begin{theorem}
%   \label{theorem:fixed-point}
%   Assume that the sequence of nonnegative learning rates obeys that $\lim_{T\rightarrow \infty}\sum_{t=0}^T
%   \eta_t  = \infty$, then 
%   $\theta\in \{\pm 1\}^d$ is a fixed point for
%   BinaryConnect~\cref{equation:batch-bc} \emph{if and only if} $\sign(\nabla
%   L(\theta)[i])=-\theta[i]$ for all $i\in[d]$ such that $\nabla
%   L(\theta)[i]\neq 0$. Such a point may not exist, in which case
%   BinaryConnect does not converge with any initialization $h_0\in \R^d$.
% \end{theorem}

We start with the ``$\Rightarrow$'' direction.
If $s$ is a fixed point, then by definition there exists $\theta_0\in\R^{d}$ such that $\theta_t = \theta$ for all $t  = 0,1,2,...$. By the iterates \cref{equation:batch-bc}
$$
\theta_T= \theta_0 - \sum_{t=0}^T \eta_t \grad L(s_t).
$$
Take signs on both sides and apply $s_t = s$ for all $t$ on both sides, we get that
$$
s = s_T  =  \sign(\theta_T) =  \sign\left(\theta_0 -   \grad L(s)  \sum_{t=0}^T \eta_t\right)
$$
Take the limit $T\rightarrow \infty$ and apply the assumption that $\sum_t \eta_t = \infty$, we get that for all $i \in [d]$ such that $[\grad L(\theta)]_i\neq 0$,  
$$
s[i]  = \lim_{T\rightarrow \infty}	\sign\left(\theta_0 -   \grad L(s)  \sum_{t=0}^T \eta_t\right)[i] =    - \sign(\grad L(s))[i].
$$

Now we prove the ``$\Leftarrow$'' direction.  If $\theta$ obeys that
$\sign(\nabla L(s)[i])=-s[i]$ for all $i\in[d]$ such that
$\nabla L(s)[i]\neq 0$, then if we take any $\theta_0$ such that
$\sign(\theta_0) = s$, $\theta_t$ will move in a straight line towards the
direction of $-\nabla L(s)$, which does not change the sign of
$h_0$. In other words, $s_t = \sign(\theta_t) = \sign(\theta_0) = s$
for all $t=0,1,2,...$.  Therefore, by definition, $s$ is a fixed
point.

%	
% Suppose $\sign(\grad L(\theta)) = -\theta$ for some
%  $\theta\in\set{\pm 1}$ and BinaryConnect reaches $\theta$ at
%  iteration $t$, i.e. $\sign(\theta_t) = \theta$, then we have
%  \begin{equation*}
%    \theta_{t+1} = \theta_t - \eta_t\grad L(\sign(\theta_t)) =
%    \theta_t - \eta_t\grad L(\theta).
%  \end{equation*}
%  As $-\eta_t\grad L(\theta)$ has the same sign as
%  $\theta=\sign(\theta_t)$, we have
%  $\sign(\theta_{t+1})=\sign(\theta_t)=\theta$, so the binarization of
%  $\theta_{t+1}$ is also $\theta$, and thus BinaryConnect converges to
%  the binarization $\theta$ (though the full-precision parameter still
%  moves).
%
%  Conversely, suppose that $\theta$ does not satisfy $\sign(\grad
%  L(\theta))=-\theta$; we argue that BinaryConnect cannot converge to
%  $\theta$. Assume the contrary, i.e. $\sign(\theta_t)=\theta$ for all
%  $t\ge T$, then we have for all $t_0\ge 1$ that
%  \begin{equation}
%    \theta_{T+t_0} = \theta_T - \sum_{t=0}^{t_0-1}\eta_{T+t}\grad
%    L(\sign(\theta_{T+t})) = \theta_T -
%    \sum_{t=0}^{t_0-1}\eta_{T+t}\grad L(\theta).
%  \end{equation}
%  As the sign of $-\grad L(\theta)$ is not equal to $\theta$ and
%  $\sum_{t\ge 0} \eta_{T+t}=\infty$, the sign of the right hand side
%  will eventually change, which means that for some $t_0$ we have
%  $\sign(\theta_{T+t_0})\neq \sign(\theta_T)=\theta$, a
%  contradiction. Therefore BinaryConnect will not stay at $\theta$.
